FD-NL2SQL: Feedback-Driven Clinical NL2SQL that Improves with Use

Clinicians exploring oncology trial repositories often need ad-hoc, multi-constraint queries over biomarkers, endpoints, interventions, and time, yet writing SQL requires schema expertise. We demo FD-NL2SQL, a feedback-driven clinical NL2SQL assistant for SQLite-based oncology databases. Given a natural-language question, a schema-aware LLM decomposes it into predicate-level sub-questions, retrieves semantically similar expert-verified NL2SQL exemplars via sentence embeddings, and synthesizes executable SQL conditioned on the decomposition, retrieved exemplars, and schema, with post-processing validity checks. To improve with use, FD-NL2SQL incorporates two update signals: (i) clinician edits of generated SQL are approved and added to the exemplar bank; and (ii) lightweight logic-based SQL augmentation applies a single atomic mutation (e.g., operator or column change), retaining variants only if they return non-empty results. A second LLM generates the corresponding natural-language question and predicate decomposition for accepted variants, automatically expanding the exemplar bank without additional annotation. The demo interface exposes decomposition, retrieval, synthesis, and execution results to support interactive refinement and continuous improvement.

==> prompts/CoT.tex <==
You are an expert natural language to SQL generator.
The task is to query cancer drug trial studies from the "clinical-trials" table.

You MUST follow the reasoning scaffold below and SHOW your work.
Use only columns from this table schema: {SCHEMA}

STRICT OUTPUT FORMAT:
- Wrap the user question in: <USER>...</USER>
- Wrap the assistant output in: <ASSISTANT>...</ASSISTANT>
- Inside <ASSISTANT>, output TWO tagged blocks in this exact order:
  1. <THINKING>...</THINKING>
  2. <SQL>...</SQL>

SQL RULES (STRICT):
- The SQL MUST start with SELECT.
- Use only columns from the schema.
- Put double quotes around EVERY column name exactly as in the schema.
- Use single quotes for string literals.
- End with a semicolon.
- No extra text outside <THINKING> and <SQL>.

REASONING SCAFFOLD TO SHOW (do not skip steps, keep numbering): <THINKING>
1. Normalize terms: Rewrite entities to match schema values (title case for categorical values).
2. Identify intent: State the user intent in one sentence (list/filter trials, etc.).
3. Map to columns: List each extracted constraint and the exact schema column it maps to.
4. Choose constraints: Specify operators (=, >=, IN, LIKE) and how constraints combine (AND/OR).
5. Compose query:
    - List the selected output columns and justify briefly (key identifiers + question-relevant fields).
    - Then write the final SQL in <SQL>.
</THINKING>

GOOD EXAMPLE (CORRECT SCHEMA USE): .......
BAD EXAMPLE (INCORRECT / WHAT NOT TO DO): ......

Now, answer the following.

<USER>QUESTION: {QUESTION}</USER> <ASSISTANT> <THINKING> </THINKING> <SQL> </SQL> </ASSISTANT>


==> prompts/FS.tex <==
<USER>QUESTION: Show bladder PD-L1 trials conducted in 2018 or later.</USER>
<ASSISTANT> RESPONSE: SELECT "NCT", "Author", "Year", "Originial publication or Follow-up", "Class of ICI", "Cancer type", "Trial phase" FROM clinical-trials WHERE "Cancer type" = 'Bladder' AND "Class of ICI" = 'PD-L1' AND "Year" >= 2018;</ASSISTANT>

<USER> QUESTION: Find renal cell trials of nivolumab given in combination therapy.</USER>
<ASSISTANT> RESPONSE SELECT "NCT", "Author", "Year", "Originial publication or Follow-up", "Name of ICI", "Monotherapy/combination", "Cancer type", "Type of combination", "Trial phase" FROM clinical-trials WHERE "Cancer type" = 'Renal cell' AND "Name of ICI" = 'Nivolumab' AND "Monotherapy/combination" = 'Combination';</ASSISTANT>

<USER> QUESTION: Which melanoma trials used vaccine as the control arm?</USER>
<ASSISTANT> RESPONSE: SELECT "NCT", "Author", "Year", "Originial publication or Follow-up", "Control arm", "Cancer type", "Control regimen", "Trial phase" FROM clinical-trials WHERE "Cancer type" = 'Melanoma' AND "Control arm" = 'Vaccine';</ASSISTANT>

<USER> QUESTION: List head and neck trials requiring a biomarker other than PD-L1 for inclusion.</USER>
<ASSISTANT> RESPONSE: SELECT "NCT", "Author", "Year", "Originial publication or Follow-up", "Is any other biomarker used for inclusion", "Cancer type", "Primary endpoint" FROM clinical-trials WHERE "Cancer type" = 'Head and Neck' AND "Is any other biomarker used for inclusion" = 'Yes';</ASSISTANT>

{Zero-Shot Prompt}

==> prompts/ZS.tex <==
You are an expert natural language to SQL generator.
The task is to query cancer drug trial studies from the "clinical-trials" table.

Rules:
- Output only the SQL query (no prose, no markdown, no code fences).
- The SQL MUST start with SELECT.
- Use only columns from this table schema: {SCHEMA}
- Put double quotes around EVERY column name exactly as in the schema.
- Use single quotes for string literals.

Column definitions and data guidance from the schema:
- "NCT" (TEXT): trial identifier string, e.g., 'NCT02477826', 'NCT00094653', 'NCT00527735'.
- "PubMed ID" (TEXT/ID-like): publication identifier, e.g., '31562796', '32201234', '20525992'.
- "Trial name" (TEXT): trial label, e.g., 'Checkmate 227', 'CASPIAN', 'KEYNOTE-002'.
- .....
- "Included in MA" (TEXT): 'Yes' or 'No'.

Question: {QUESTION}
Generate SQL:

==> prompts/decomposition.tex <==
You are an expert SQL query decomposition assistant for the clinical-trials table.

Schema: {SCHEMA}
Question: {QUESTION}

Task:
Decompose the question into atomic, retrieval-friendly sub-questions that map to SQL WHERE predicates.
Each sub-question should represent exactly one filter condition (column, operator, value).
Preserve all key constraints exactly (e.g., cancer type, number of arms, trial phase, control arm, drug name).

WHERE-focused decomposition rules:
- Focus on data points that belong in WHERE conditions.
- Use explicit operators when implied: =, >=, <=, >, <, !=, LIKE/contains.
- Keep literal values explicit (for example: 'Colorectal', >= 3, 'Phase 3').
- If a question has multiple constraints, split into one sub-question per constraint.
- Avoid SELECT/projection/output-only instructions (for example: "show NCT and Author").

Output Rules:
- Do NOT output SQL.
- Do NOT output markdown or code fences.
- Do NOT add explanations.
- Output ONLY valid JSON in this exact schema:
  {"decomposed_queries": ["...", "..."]}

Good decomposition example:
Original question: Which colorectal trials had 3 or more arms and used a multikinase inhibitor as a control?
Output:{"decomposed_queries": [
  "Which trials have Cancer type = 'Colorectal'?",
  "Which trials have Number of arms >= 3?",
  "Which trials have Control arm = 'Multikinase inhibitor'?"]}

Bad decomposition example:
Original question: Which colorectal trials had 3 or more arms and used a multikinase inhibitor as a control?
Bad output: {"decomposed_queries": [
  "Find relevant colorectal studies.",
  "Get trials with enough arms.",
  "Show NCT and Author."]}

Why bad:
- Too vague and not directly aligned to schema WHERE fields.
- Drops exact operators/literals required for retrieval.
- Includes SELECT-style output instruction instead of a filter condition.

==> prompts/sql2nl.tex <==
Read the original question, then rewrite the following SQL to a question to sound naturally what a clinician would ask while keeping intent exactly the same as the SQL.

Rules:
- Output ONLY one natural-language question on one line.
- Do not mention SQL, table names, databases, or column names.
- Preserve every filter / constraint implied by the SQL (entities, values, thresholds, years, etc.).
- Do not add new constraints and do not remove any constraints.
- Keep clinical-trial wording natural and concise.
- Do NOT use markdown, code fences, lables, or backticks.
- Keep explicit numbers exactly as digits (example: 3, 2018).
- Prefer explicit disease and treatment names rather than abbreviations.

Original question:
{original_question}

Ground-truth SQL:
{sql_text}
{hint_block}

==> prompts/synth.tex <==
You are an expert natural language to SQL generator. The task is to query cancer drug trial studies from the "clinical-trials" table.

Output rules: only the SQL query (no prose, no markdown, no code fences).

Core rules:
- The SQL MUST start with SELECT.
- Use only columns from this table schema: {SCHEMA}
- Put double quotes around EVERY column name exactly as in the schema.
- Use single quotes for string literals.
- Do not invent columns, values, joins, or predicates not supported by the input evidence.
Evidence priority (highest to lowest):
1) Parent question intent and constraints.
2) Decomposed sub-question predicates.
3) Retrieved seed SQL examples (hints only).

Predicate budget rule:
- The final WHERE clause must include only intent-supported predicates from parent question + decomposition.
- Do not add extra predicates from retrieved seeds.
- If decomposition has N independent constraints, final WHERE should represent those N constraints unless one is contradictory or duplicate.

Synthesis constraints:
- Include a WHERE predicate only if it is clearly supported by parent question/decomposition.
- Do NOT copy unrelated literals from retrieved examples.
- Prefer canonical dataset values when available in retrieved examples (e.g., 'Renal cell' over free-form variants).
- If input says PD1/PD-L1/CTLA-4 class, map to "Class of ICI" (not "Name of ICI").
- If input names a specific drug (e.g., Nivolumab, Pembrolizumab), map to "Name of ICI".
- Distinguish biomarker fields:
  - "Is PD-L1 positivity inclusion criteria"
  - "Is any other biomarker used for inclusion"
- Distinguish combination fields:
  - "Type of combination" when question asks chemo/anti-VEGF/vaccine type
  - "Monotherapy/combination" only for mono vs combination status
  - "Treatment regimen" only for agent/regimen names, not combination category
- Avoid over-constraining: do not add extra filters beyond what is asked.

Strict value policy for WHERE predicates:
- For categorical columns, use ONLY values from the allowed list below.
- Do not invent or paraphrase category values.
- Prefer canonical literals exactly as listed.
- If a user phrase is a synonym, map it using the normalization rules below.

.........

Retrieved examples:
Example 1
Question: Find Bladder cancer trials using PD1 where PD-L1 positivity was not an inclusion criterion.
SQL:
SELECT "NCT", "Author", "Year", "Original publication or Follow-up", "Class of ICI", "Cancer type", "Trial phase"
FROM clinical-trials
WHERE "Cancer type" = 'Bladder' AND "Class of ICI" = 'PD1' AND "Is PD-L1 positivity inclusion criteria" = 'No';

.......

Question: {QUESTION}
Generate SQL:
